A transmission hologram for slitless spectrophotometry on a convergent telescope beam. 1. Focus and resolution

We report in this paper the test of a plane holographic optical element to be used as an aberration-corrected grating for a slitless spectrograph, inserted in a convergent telescope beam. Our long term objective is the optimisation of a specific hologram to switch the auxiliary telescope imager of the Vera Rubin Observatory into an accurate slitless spectrograph, dedicated to the atmospheric transmission measurement. We present and discuss here the promising results of tests performed with prototype holograms at the CTIO $0.9\,$m telescope during a run of 17 nights in May-June 2017. After their on-sky geometrical characterisation, the performances of the holograms as aberration-balanced dispersive optical elements have been established by analysing spectra obtained from spectrophotometric standard stars and narrow-band emitter planetary nebulae. Thanks to their additional optical function, our holographic disperser prototypes allow to produce significantly better focused spectra within the full visible wavelength domain $[370,1050]\,$nm than a regular grating, which suffers from strong defocusing and aberrations when used in similar conditions. We show that the resolution of our slitless on-axis spectrograph equipped with the hologram approaches its theoretical performance. While estimating the benefits of an hologram for the spectrum resolution, the roadmap to produce a competitive holographic element for the Vera Rubin Observatory auxiliary telescope has been established.

==> Makefile <==

# Makefile (L. Le Guillou, 2020-09-01)

LATEX = latex
PDFLATEX = pdflatex
DVIPS = dvips
DVIPDF = dvipdf -sPAPERSIZE=a4
PS2PDF = ps2pdf
BIBTEX = bibtex
MAKEINDEX = makeindex

PSSELECT = psselect

MV = mv -f
RM = rm -f


TEXFILES = main.tex

BIBFILES = citations_holospec.bib

# -- Thesis ----------------------------------------------------------

all:	paper-holospec1.pdf

paper-holospec1.pdf:	$(TEXFILES) $(BIBFILES)
			$(PDFLATEX) main.tex
			$(PDFLATEX) main.tex
			$(BIBTEX) main
			$(PDFLATEX) main.tex
			$(PDFLATEX) main.tex
			$(PDFLATEX) main.tex
			$(MV) main.pdf paper-holospec1.pdf

# --------------------------------------------------------------------

clean:
		$(RM) *.toc *.aux *.lot *.lof \
                      *.bbl *.blg *.idx *.ilg *.ind *.out \
		      *.log *.dvi *.ps.* paper-holospec1.pdf

# --------------------------------------------------------------------


